"A Nova Eletricidade: Aplica\c{c}\~oes, Riscos e Tend\^encias da IA Moderna -- "The New Electricity": Applications, Risks, and Trends in Current AI

The thought-provoking analogy between AI and electricity, made by computer scientist and entrepreneur Andrew Ng, summarizes the deep transformation that recent advances in Artificial Intelligence (AI) have triggered in the world. This chapter presents an overview of the ever-evolving landscape of AI, written in Portuguese. With no intent to exhaust the subject, we explore the AI applications that are redefining sectors of the economy, impacting society and humanity. We analyze the risks that may come along with rapid technological progress and future trends in AI, an area that is on the path to becoming a general-purpose technology, just like electricity, which revolutionized society in the 19th and 20th centuries. A provocativa compara\c{c}\~ao entre IA e eletricidade, feita pelo cientista da computa\c{c}\~ao e empreendedor Andrew Ng, resume a profunda transforma\c{c}\~ao que os recentes avan\c{c}os em Intelig\^encia Artificial (IA) t\^em desencadeado no mundo. Este cap\'itulo apresenta uma vis\~ao geral pela paisagem em constante evolu\c{c}\~ao da IA. Sem pretens\~oes de exaurir o assunto, exploramos as aplica\c{c}\~oes que est\~ao redefinindo setores da economia, impactando a sociedade e a humanidade. Analisamos os riscos que acompanham o r\'apido progresso tecnol\'ogico e as tend\^encias futuras da IA, \'area que trilha o caminho para se tornar uma tecnologia de prop\'osito geral, assim como a eletricidade, que revolucionou a sociedade dos s\'eculos XIX e XX.

==> sections/jogos.tex <==
\section{Jogos}
\label{sec:jogos}
% by chatgpt:
Inteligência Artificial (IA) tornou-se uma ferramenta indispensável no domínio dos jogos, revolucionando a indústria de jogos ao aprimorar as experiências dos jogadores, permitir a geração de conteúdo dinâmico e otimizar os processos de desenvolvimento de jogos. 

\subsection{Aplicações}

\subsection{Riscos}
Atualmente, há um grande debate global sobre os impactos e riscos da IA na economia e sociedade, bem como em temas específicos, como as consequências da IA no mercado de trabalho \cite{nature-ethics}. Notadamente, governos das nações líderes em IA, como EUA, China e Reino Unido, bem como esforços coletivos da União Europeia e organismos como Organização para a Cooperação e Desenvolvimento Econômico (OECD)\footnote{\url{https://oecd.ai/en/ai-principles} Employment Outlook 2023: Artificial Intelligence and the Labour Market, 11 Jul 2023  OECD, 267 pages.  Acesso em 08 de Agosto de 2023.}, Fórum Econômico Mundial (WEF)\footnote{\url{https://www.weforum.org/agenda/2023/07/ai-biggest-risks-how-to-manage-them/} AI: These are the biggest risks to businesses and how to manage them. Jul 27, 2023. Acesso em 08 de Agosto de 2023.}  
e Nações Unidas\footnote{\url{https://press.un.org/en/2023/sgsm21880.doc.htm} 18 July 2023: Secretary-General Urges Security Council to Ensure Transparency, Accountability, Oversight, in First Debate on Artificial Intelligence. Acesso em 08 de Agosto de 2023} têm constituído grupos de trabalho para identificar, compreender e tentar predizer os riscos da aplicação das tecnologias de IA.
Após o recente impacto na mídia do modelo de linguagem ChatGPT \footnote{\url{https://openai.com/blog/chatgpt}} lançado em Novembro de 2022, a IA tornou-se assunto de todos os canais de comunicação, com inúmeros especialistas e leigos opinando sobre o assunto. Governos imediatamente, às vezes às pressas, organizaram grupos de trabalho, reunindo pessoas para analisar tais impactos. Aqui, reside um dos primeiros riscos que identificamos no atual debate: a influência construída sobre a opinião pública justamente a partir de opiniões leigas - de pessoas que têm pouca ou nenhuma experiência em desenvolvimento de tecnologias de IA - tampouco conhecimento dos fundamentos científicas da área. Isto impõe sérios riscos à sociedade, criando situação análoga à da recente pandemia da COVID-19, na qual leigos opinavam sobre o uso de medidas sanitárias, gerando dúvidas para a população, levando os governos e, consequentemente, a gestão da pandemia a um ambiente de ainda maior risco e insegurança decisória. No momento atual, em que a IA chama a atenção de todos, devemos alertar para a necessidade de consultarmos especialistas no assunto. Estes especialistas são aqueles que de fato trabalham na área, profissionalmente desenvolvendo tecnologias ou nos centros de pesquisas acadêmicos e empresariais \emph{na área de inteligência artificial}. 


\subsection{Tendências}

==> sections/neurosimb.tex <==
% Movido p/ subsecao na conclusao -- aqui nao precisou comentar, bastou comentar o \input no main.tex
\section{IA Neuro-simbólica}
\label{sec:neurosimb}
%%Begin Lamb escreveu
A IA iniciou sua trajetória buscando a integração entre diversas habilidades cognitivas, dentre elas, o raciocínio e o aprendizado. Ambas dimensões são vistas como centrais à ideia de inteligência de máquina, já nos trabalhos originais de Turing, von Neumann, McCulloch, Pitts, entre outros \cite{turing1950}. von Neumann, em seus trabalhos iniciais, já identificava a relação entre a lógica intuicionista \cite{von1956probabilistic,GarcezLG06} e as redes neurais propostas por \cite{McCulloch1943}.\footnote{von Neumann foi explícito ao identificar a relação entre a lógica intuicionista e os modelos de rede neural de \cite{McCulloch1943}. Na seção 2 de \cite{von1956probabilistic}, von Neumann afirma que "It has been pointed out by A. M. Turing [5] in 1937 and by W. S. McCulloch and W. Pitts [2] in 1943 that effectively constructive logics, that is, intuitionistic logics, can be best studied in terms of automata. Thus logical propositions can be represented as
electrical networks or (idealized) nervous systems." As referências [5] e [2] nesta citação são, respectivamente:  A. M. Turing “On computable numbers,” Proc. of the London Math. Soc. 2-42(1937), p. 230-265 e W. S. McCulloch and W. Pitts, “A logical calculus of the ideas imminent in nervous activity,” Bull. of Math. Biophysics, 5 (l943), p. 115-133. Mais informações sobre a evolução da IA, em particular IA neurosimbólica podem ser encontradas em \cite{Audibert2022,GarcezLG2009,3rdWave}.}

Entre leigos, confunde-se atualmente o que é IA com modelos grandes de linguagem (LLMs - large language models). No entanto, a IA vai muito além desta tecnologia específica, que apenas tangencia as demais subáreas da IA. Notadamente, modelos de linguagens têm grandes limitações, com impactos sobre os usuários no que se refere à explicabilidade (por quais razões -  e como - os modelos de linguagem geram os seus resultados), interpretabilidade (como interpretar, através de um modelo semanticamente rigoroso, o significado dos resultados, bem como a própria construção destes sistemas), vieses (resultados destes sistemas que causam prejuízo a grupos de pessoas, como viés de gênero, raça, sexo, profissão, nacionalidade, cultura, seleção para empregos, correção de provas, entre outros), além de chamadas alucinações, onde se nota que os modelos de linguagens geram resultados sem nenhuma relação com os "prompts" e interações com os usuários. 

Tais limitações apontam para técnicas de IA que venham a solucionar estes desafios, como ofereçam uma semântica, isto é, um significado para as computações realizadas pelos modelos de linguagem. Ademais, não são apenas os LLMs que carecem de uma semântica formal. Modelos de aprendizado profundo, embora tenham apresentados resultados tecnológicos relevantes, não apresentam uma semântica rigorosa (isto é, não são modelos que tenham associados uma interpretação lógico-matemática). Assim, os estudos em IA neurosimbólica visam, entre outros objetivos, oferecer interpretações (ou explicações, se a posteriori) dos métodos e mecanismos de aprendizado atualmente utilizados em IA. Mas, por qual motivo queremos uma interpretação dos modelos de aprendizado? Basicamente, do ponto de vista tecnológico (e de produto) oferecer garantias sobre o comportamento de um sistema, bem como entender exatamente porque um determinado sistema apresenta tal comportamento é um requisito básico de qualquer produto tecnológico.  

A área de IA neuro-simbólica integra os dois principais paradigmas da IA: conexionismo (notadamente associado ao uso de redes neurais artificiais como seu modelo principal) e simbolismo (onde o processo de raciocínio em IA é representado através de lógicas, incluindo diversas modalidades como tempo, espaço, conhecimento e incerteza) \cite{GarcezLG07,AAAI07,3rdWave}. Na história recente, a partir dos anos 1990, estas áreas foram desenvolvidas por correntes diversas, por terem fundamentos computacionais e lógicos distintos \cite{Besold2022,GarcezLG2009}. 
A área recebeu certa atenção inicial nos anos 1990 e 2000 \cite{hinton}, quando pesquisadores passaram a desenvolver abordagens  neuro-simbólicas que aprendessem a realizar inferência lógica clássica, mesmo que para fragmentos de lógicas de predicados \cite{Audibert2022,Garcez_1999}. À época, foram desenvolvidos sistemas neuro-simbólicos que aprendiam a computar (fragmentos) de programas escritos em linguagens lógicas, como Prolog. Posteriormente, pesquisadores demonstraram que modelos conexionistas poderiam ser treinados para aprender regras de inferência lógica, notadamente sobre lógicas não-clássicas, permitindo a expressão de multi-modalidades \cite{NIPS03,NECO3050,AAAI07}. Além disso, a adição destas modalidades, integrando raciocínio e aprendizado sobre tempo, espaço e incerteza antecipa, de certa forma, a linha de pesquisa atual em grandes modelos de linguagens que visa expressar multimodalidades na interação entre usuários e esses sistemas \cite{Kiros2014}.

As grandes contribuições que a área de IA neuro-simbólica pode oferecer são sumarizadas em artigos recentes, publicados na \emph{Communications of the ACM} \cite{Monroe2022, Hochreiter22}. Monroe ressalta a necessidade de desenvolvimento de uma semântica rigorosa para os modelos de IA, como defendido em \cite{3rdWave,LambIJCAI2020}, enquanto Hochreiter aponta que a forma de desenvolver uma IA ampla, que contemple múltiplas habilidades cognitivas, pode ser melhor atingida através da IA neurosimbólica, sugerindo a abordagem de redes grafos neurais neuro-simbólicos; Hochreiter cita especificamente o trabalho \cite{LambIJCAI2020} como sendo promissor para esta linha de pesquisa em IA ampla, que vai além dos sistemas e tecnologias atuais, que somente são focados em um dimensão cognitiva, como e.g., reconhecimento de imagens, visão computacional, ou processamento de linguagem natural. É relevante ressaltar que esta necessidade de integração neuro-simbólica foi apontada como promissora em eventos recentes, como nas conferências AAAI e NeurIPS, bem como nos debates organizados pela  Montreal AI, denominadas de "AI Debates"\footnote{\url{https://www.quebecartificialintelligence.com/aidebate2/}} números 1, 2 e 3.  Nestes eventos, foi apontado que para construir sistemas que representem as duas formas de raciocínio -  na forma de "AI Fast and Slow" inspirado em \cite{Kahneman2017thinking} - visando a integração de múltiplas habilidades cognitivas em IA, possíveis abordagens promissoras seriam justamente as adotadas na IA neuro-simbólica. Estas abordagens oferecem a possibilidade do desenvolvimento de modelos com fundamentação rigorosa e transparente do ponto de vista lógico, que se integrados ao aprendizado profundo podem levar a tecnologias de inteligência artificial mais robustas, explicáveis e transparentes, oferecendo maior segurança a todos que fazem uso desta tecnologia de propósito geral \cite{3rdWave}.

%2 pages
%%End Lamb escreveu.
